An Empirical Study on the Impact of Positional Encoding in Transformer-based Monaural Speech Enhancement

Transformer architecture has enabled recent progress in speech enhancement. Since Transformers are position-agostic, positional encoding is the de facto standard component used to enable Transformers to distinguish the order of elements in a sequence. However, it remains unclear how positional encoding exactly impacts speech enhancement based on Transformer architectures. In this paper, we perform a comprehensive empirical study evaluating five positional encoding methods, i.e., Sinusoidal and learned absolute position embedding (APE), T5-RPE, KERPLE, as well as the Transformer without positional encoding (No-Pos), across both causal and noncausal configurations. We conduct extensive speech enhancement experiments, involving spectral mapping and masking methods. Our findings establish that positional encoding is not quite helpful for the models in a causal configuration, which indicates that causal attention may implicitly incorporate position information. In a noncausal configuration, the models significantly benefit from the use of positional encoding. In addition, we find that among the four position embeddings, relative position embeddings outperform APEs.

==> data/com.tex <==
\renewcommand\arraystretch{1.0}
\vspace{-1.0em}
\begin{table}[!hbpt]
\centering
    \scriptsize
    \def\arraystretch{1.2}
    \setlength{\tabcolsep}{2.3pt}
\caption{Average scores of CSIG, CBAK, and COVL across all test conditions. The highest scores are highlighted in boldface.}
\label{tabwer}
\vspace*{0.1in}
\scalebox{1}{
\begin{tabular}{l|ccc|ccc }
\toprule
\multirow{2}{*}{\textbf{Network}}  & \multicolumn{3}{c|}{\textbf{IRM}} & \multicolumn{3}{c}{\textbf{PSM}}  \\
\cline{2-7}
 &  \textbf{CSIG} & \textbf{CBAK} & \textbf{COVL} & \textbf{CSIG} & \textbf{CBAK} & \textbf{COVL} \\
\toprule 
Noisy & 2.26  & 1.80  & 1.67  & - & - & -  \\
\toprule   
% \textbf{GaResTCN}       
%  & 3.15 & 2.48 & 2.42 & 3.15 & 2.51 & 2.45 \\
ResTCN+SA \cite{restcnsa}     
& 3.10 & 2.45 & 2.37 & 3.14 & 2.53 & 2.46 \\
MHANet \cite{mhanet}      
& 3.13 & 2.46 & 2.40 & 3.21 & 2.56 & 2.51 \\
\toprule 
ResTCN \cite{deepmmse}     
& 3.08 & 2.43 & 2.35 & 3.12 & 2.52 & 2.44 \\
ResTCN+FA    
& 3.21 & 2.51 & 2.48 & 3.25 & 2.61 & 2.55 \\      
ResTCN+TA       
& 3.23 & 2.53 & 2.49 & 3.27 & 2.58 & 2.57 \\
ResTCN+TFA    
& \textbf{3.28} &\textbf{2.56} & \textbf{2.54} & \textbf{3.33} & \textbf{2.64} & \textbf{2.62} \\  
% \midrule[0.8pt]
% \midrule[0.8pt]
% ResMLP      & 2.60  & 2.14 & 1.95 & 2.64 & 2.18 & 2.00 \\
% ResMLP+TFA  & \textbf{2.95} & \textbf{2.31} & \textbf{2.23} & \textbf{2.95} & \textbf{2.39} & \textbf{2.28} \\
\toprule  
\end{tabular}}
\label{composite}
\vspace{-2em}
\end{table}

==> data/estoi.tex <==
\begin{table}[!htbp]
    % \vspace{-1.0em}
    \centering
    \scriptsize
    \def\arraystretch{1.2}
    \setlength{\tabcolsep}{4.5pt}
    \footnotesize	
    \caption{Average ESTOI scores (in \%) for each SNR level. The highest ESTOI scores are highlighted in boldface.}
    \label{tabwer}
    \vspace{1.5in}
    \scalebox{0.90}{\begin{tabular}{clrccccc}
        \toprule
        & & & \multicolumn{5}{c}{\textbf{Input SNR (dB)}}\\  
        \cmidrule[0.8pt]{4-8}
        \textbf{Target} & \textbf{Network} & {\textbf{\# Params}} & -5 & 0 & 5 & 10 & 15 \\
        \toprule
        - & Noisy & & 27.91 & 42.14 & 57.21 & 71.11 & 82.22 \\
        \toprule
        \multirow{5}{*}{\textbf{IRM}}
        % & ResLSTM & 43.16 & 59.80 & 73.16 & 82.74 & 89.25  \\
        % & CRN & 43.97 & 61.27 & 74.40 & 83.39 & 89.55  \\
        % & GaResTCN   & 3.78M & 43.02 & 60.70 & 74.53 & 83.80 & 89.79  \\
        & ResTCN+SA \cite{restcnsa}    & 2.24M & 43.32 & 60.68 & 74.37 & 83.67 & 89.77  \\
        & MHANet \cite{mhanet}       & 4.08M & 43.72 & 61.08 & 74.68 & 83.90 & 89.96  \\
        \cmidrule[0.8pt]{2-8}
        & ResTCN \cite{deepmmse}       & 1.98M  & 42.47 & 59.93 & 73.67 & 83.22 & 89.44  \\
        & ResTCN+FA    & +1.36K & 44.87 & 61.73 & 75.06 & 84.27 & 90.09\\
        & ResTCN+TA    & +1.36K & 46.11 & 62.96 & 75.86 & 84.48 & 90.21\\
        & ResTCN+TFA   & +2.72K & \textbf{47.61} & \textbf{64.05} & \textbf{78.61} & \textbf{85.45} & \textbf{90.83}\\
        % \cmidrule[0.8pt]{2-8}
        % & ResMLP        & 1.58M  & 31.76 & 48.39 & 64.36 & 77.04 & 85.71 \\
        % & ResMLP+TFA    & +0.34K & \textbf{38.14} & \textbf{55.39} & \textbf{70.11} & \textbf{81.08} & \textbf{88.33} \\
        \toprule
        \toprule
        
        \multirow{5}{*}{\textbf{PSM}}
        % & ResLSTM & 42.73 & 60.11 & 74.02 & 83.55 & 89.84  \\
        % & CRN & 44.51 & 62.74 & 75.98 & 84.73 & 90.38  \\
        % & GaResTCN   & 3.78M & 42.77 & 60.75 & 74.58 & 84.05 & 90.01  \\
        & ResTCN+SA \cite{restcnsa}    & 2.24M & 43.03 & 61.13 & 75.07 & 84.24 & 90.07  \\
        & MHANet \cite{mhanet}       & 4.08M & 44.66 & 62.32 & 75.74 & 84.69 & 90.43  \\
        \cmidrule[0.8pt]{2-8}
        & ResTCN \cite{deepmmse}       & 1.98M  & 42.76 & 60.45 & 74.47 & 83.91 & 89.84  \\
        & ResTCN+FA    & +1.36K & 44.91 & 62.38 & 75.88 & 84.82 & 90.45\\
        & ResTCN+TA    & +1.36K & 45.70 & 63.25 & 76.49 & 85.09 & 90.70\\
        & ResTCN+TFA   & +2.72K & \textbf{48.67} & \textbf{65.28} & \textbf{77.43} & \textbf{85.80} & \textbf{91.16}\\

        \bottomrule
    \end{tabular}}
    \label{estoi}
    % \vspace{-0.5em}
\end{table}

==> data/pesq.tex <==
\begin{table}[!h]
    % \vspace{-1.0em}
    \centering
    \scriptsize
    \def\arraystretch{1.2}
    \setlength{\tabcolsep}{4.5pt}
    \footnotesize	
    \caption{Average PESQ (wideband version) scores for each SNR level. The highest PESQ scores are highlighted in boldface.}
    \label{tabwer}
    % \vspace*{0.5em}
    \scalebox{0.92}{\begin{tabular}{clrccccc}
        \toprule
        &  &  & \multicolumn{5}{c}{\textbf{Input SNR (dB)}}\\  
        \cmidrule[0.8pt]{4-8}
        {\textbf{Target}} & {\textbf{Network}} & {\textbf{\# Params}} & -5 & 0 & 5 & 10 & 15 \\
        \toprule
        - & Noisy & & 1.05 & 1.07 & 1.13 & 1.31 & 1.64 \\
        \toprule
        \multirow{5}{*}{\textbf{IRM}}
        % &  GaResTCN \cite{grn}       & 3.78M & 1.15 & 1.36 & 1.68 & 2.12 & 2.58  \\
        & ResTCN+SA \cite{restcnsa} & 2.24M & 1.15 & 1.34 & 1.64 & 2.07 & 2.51  \\
        & MHANet \cite{mhanet}      & 4.08M & 1.16 & 1.36 & 1.68 & 2.10 & 2.56  \\
        \cmidrule[0.8pt]{2-8}
        & ResTCN 
        \cite{deepmmse} & 1.98M  & 1.13 & 1.32 & 1.61 & 2.06 & 2.50  \\
        & ResTCN+FA     & +1.36K & 1.18 & 1.39 & 1.74 & 2.15 & 2.60 \\
        & ResTCN+TA     & +1.36K & 1.18 & 1.40 & 1.75 & 2.19 & 2.63 \\
        & ResTCN+TFA    & +2.72K & \textbf{1.20} & \textbf{1.43} & \textbf{1.79} & \textbf{2.27} & \textbf{2.70}\\
        % \cmidrule[0.8pt]{2-8}
        % & ResMLP        & 1.58M  & 1.07 & 1.15 & 1.33 & 1.62 & 2.03 \\
        % & ResMLP+TFA    & +0.34K & \textbf{1.11} & \textbf{1.26} & \textbf{1.51} & \textbf{1.90} & \textbf{2.38} \\
        \toprule
        \toprule
        
        \multirow{5}{*}{\textbf{PSM}}
        % & GaResTCN \cite{grn}       & 3.78M & 1.18 & 1.41 & 1.77 & 2.24 & 2.72  \\
        & ResTCN+SA \cite{restcnsa} & 2.24M & 1.20 & 1.42 & 1.79 & 2.26 & 2.75  \\
        & MHANet \cite{mhanet}      & 4.08M & 1.20 & 1.44 & 1.83 & 2.30 & 2.78  \\
        \cmidrule[0.8pt]{2-8}
        & ResTCN \cite{deepmmse}    & 1.98M & 1.19 & 1.40 & 1.76 & 2.23 & 2.72  \\
        & ResTCN+FA   & +1.36K & 1.20 & 1.47 & 1.87 & 2.36 & 2.85\\
        & ResTCN+TA   & +1.36K & 1.21 & 1.49 & 1.90 & 2.38 & 2.85\\
        & ResTCN+TFA   & +2.72K & \textbf{1.26} & \textbf{1.54} & \textbf{1.96} & \textbf{2.44} & \textbf{2.91}\\
        \bottomrule
    \end{tabular}}
    \label{pesq}
    % \vspace{-1.5em}
\end{table}
